Finding optimal Pulse Repetion Intervals with Many-objective Evolutionary Algorithms

In this paper we consider the problem of finding Pulse Repetition Intervals allowing the best compromises mitigating range and Doppler ambiguities in a Pulsed-Doppler radar system. We revisit a problem that was proposed to the Evolutionary Computation community as a real-world case to test Many-objective Optimization algorithms. We use it as a baseline to compare several Evolutionary Algorithms for black-box optimization with different metrics. Resulting data is aggregated to build a reference set of Pareto optimal points and is the starting point for further analysis and operational use by the radar designer.

==> toggledraftmode.tex <==
 % make it simpler to switch to draft, without going to the top in the main document
\renewcommand{\isdraft}{\boolean{false}}
\providecommand{\del}[2][]{}
%\renewcommand{\isdraft}{\boolean{true}}
